With arms wide open: a VLT/MUSE view of the mechanisms driving unwinding spiral arms in cluster galaxies

The environmental mechanisms driving unwinding spiral arms in cluster galaxies remain debated. While earlier studies attributed it mainly to gravitational interactions, recent works suggest that RPS alone can induce unwinding. We present a VLT/MUSE spatially resolved analysis to investigate the mechanisms responsible for spiral-arm unwinding in two galaxies, UG101 and UG103, drawn from a larger sample. They are selected as tidal and RPS-driven candidates, respectively, based on the proximity of close neighbors. We estimate the galactocentric radius at which tidal forces, from a companion or the cluster potential, become relevant ($R_{\mathrm{tid}}$). We examine gas and stellar kinematics, exploiting their different responses to gravitational and hydrodynamical perturbations. SINOPSIS is used to map stellar populations in age bins and constrain unwinding timescales. For UG101, we find $R_{\mathrm{tid}} \sim 1.5 R_e$, while the unwound features extend beyond this radius. UG101 shows irregular stellar and gas kinematics; its rotation curve indicates similar motions, although the gas is truncated on one side and extended on the other. For UG103, neither the closest companion nor the cluster appear capable of triggering unwinding. UG103 displays regular stellar but disturbed gas kinematics, with truncation on the disk side likely facing the ICM wind and gas extended in the opposite direction. Stellar population maps show the emergence and unwinding of the spiral arms in UG103 on timescales consistent with its cluster infall time ($\sim 1.6$ Gyr). We conclude that unwinding in UG101 and UG103 is primarily driven by tidal interactions and RPS, respectively, although a combined effect cannot be excluded for UG101. Our methodology provides a framework to identify the mechanisms driving unwinding in cluster galaxies from spatially resolved properties.

==> TABLES/galaxy_properties.tex <==
\begin{tabular}{llll}
\toprule
\toprule
\textbf{Property} & \textbf{UG101} & \textbf{UG101b} & \textbf{UG103} \\
\midrule
$z$ &
$0.04548 \pm 4.6\times10^{-5}$ &
$0.04871 \pm 4.6\times10^{-5}$ &
$0.05387 \pm 4.7\times10^{-5}$ \\

RA (ICRS)\tablefootmark{a} &
13:27:16.67 &
13:27:14.61 &
13:27:03.41 \\

DEC (ICRS) &
-31:49:14.67 &
-31:49:24.24 &
-31:13:31.49 \\

$z_{\rm cl}$\tablefootmark{b} &
0.04829 & 
0.04829 & 
0.04829 \\

$\sigma_{\rm cl}$\,[\si{\kilo\metre\per\second}] &
$910^{+44}_{-46}$ &
$910^{+44}_{-46}$ &
$910^{+44}_{-46}$ \\

$\log (M_{\bigstar}/M_\odot)$ &
$9.94^{+0.05}_{-0.08}$ &
$9.90^{+0.03}_{-0.06}$ &
$10.80^{+0.04}_{-0.04}$ \\

$\mathrm{SFR}$ [$M_{\odot}/\mathrm{yr}$]\tablefootmark{c} &
$0.77 \pm 0.08$ &
$(9.1 \pm 0.9)\times10^{-3}$ &
$2.4 \pm 0.2$ \\

$R_e$ [kpc] &
$5.2 \pm 0.4$ &
$1.75 \pm 0.07$ &
$8.9 \pm 0.6$ \\

PA [$^\circ$] &
$90.8 \pm 2.1$ &
$39.8 \pm 0.6$ &
$160.0 \pm 1.4$ \\

$i$ [$^\circ$] &
$42.5 \pm 1.1$ &
$41.7 \pm 0.3$ &
$34.4 \pm 1.2$ \\
\bottomrule
\end{tabular}

